The Avian Compass can be Sensitive even without Sustained Quantum Coherence

Theoretical studies indicating the presence of long-lived coherence in the radical pair system have engendered questions about the utilitarian role of sustained coherence in the avian compass. In this manuscript, we investigate this for a realistic multi-nuclear radical pair system, along with the related question of its sensitivity to the geomagnetic field. Firstly, we find that sustenance of long-lived coherence is unlikely in a realistic hyperfine environment. Secondly, probing the role of the hyperfine interactions on the compass sensitivity, we establish the hyperfine anisotropy as an essential parameter for the sensitivity. Thereby, we are able to identify a parameter regime where the compass would exhibit sensitivity even without sustained coherence.

==> Figures.tex <==
\begin{figure}[htbp]
\includegraphics[scale = 0.2]{RP_MultiNuclei.png}
\caption{Electrons Coupled to various nuclei via Hyperfine Couplings. We consider hyperfine couplings from multiple nuclei in order to account for a realistic picture of Radical pair model of Avian Magnetoreception.}
\end{figure}
\textcolor{red}{An illustration of the multi nuclei RP system.}

\begin{figure}
\includegraphics[scale = 0.7]{Figure2a.png}
\includegraphics[scale = 0.5]{Figure2b_2d.pdf}
\caption{Effect of including isotropic hyperfine interactions by increasing the number of nuclear spins that are coupled to the electron spins. 
Fig. 2a) Illustrative representation of Coherence Dynamics of Radical pair system with Multiple Nuclei Coupled via hyperfine interaction.
Fig2b) Decrease in Sensitivities as we include Isotropic Hyperfine interaction into consideration.}
\end{figure}
\textcolor{red}{Question reagrding fig 2a: The z-axis is coherence dynamics or the sensitivity?}

\textcolor{red}{Question reagrding the inference: Is the drop in sensitivity a consequence of increment in number of nuclei or a consequence of increasing isotropy?}

\begin{figure}
\centering
\includegraphics[scale = 0.6]{Figure3a.pdf}
\includegraphics[scale = 0.6]{Figure3b_2d.pdf}
\includegraphics[scale = 0.4]{Figure3c.pdf}
\caption{Coherence dynamics curves for 3-3 system with varying axial hyperfine component.\\
Fig 3a Effect of Isotropic hyperfine component on the Coherence dynamics of the system.\\
Fig3b and 3c Effect of Isotropic Hyperfine on the Singlet yields and Sensitivities.
\\ Inference : As claimed by Gauger et. al. and others, the role of sustained coherence might not be a requirement for a Sensitive Compass to function. Emphasizing the point that we achieve better sensitivities in presence of the  isotropic hyperfine components is an indication of the3}
\end{figure}

\textcolor{red}{[Question: Is $A_x$ the axial hyperfine constant?]}

\begin{figure}
\centering
\includegraphics[scale = 0.6]{Figure4a.pdf}
\includegraphics[scale = 0.6]{Figure4b_2d.pdf}
\includegraphics[scale = 0.4]{Figure4c.pdf}
\caption{Sensitivities with $\mathcal{A}_x$ change for 2-2 system}
\end{figure}
\begin{figure}
\centering
\includegraphics[scale = 0.6]{Figure5a.pdf}
\includegraphics[scale = 0.6]{Figure5b_2d.pdf}
\caption{Sensitivities with the change of recombination rates}
\end{figure}

\section{Conclusions from the figures}
\begin{itemize}
\item Figure 2 : Due to isotropic hyperfine coupling, the coherence will not be sustained and would depend on the couplings and the size of the nuclear environment.(Will give the semi - analytical arguments here)
\item The good sensitivity of the compass is the result of anisotropy in the hyperfine interaction although might  actually be dependant on $A_x (or A_y)$ components also. 
\item \textcolor{red}{What is the conclusion from Fig. 5?}
\end{itemize}
